AccaSim: a Customizable Workload Management Simulator for Job Dispatching Research in HPC Systems

We present AccaSim, a simulator for workload management in HPC systems. Thanks to AccaSim's scalability to large workload datasets, support for easy customization, and practical automated tools to aid experimentation, users can easily represent various real HPC systems, develop novel advanced dispatchers and evaluate them in a convenient way across different workload sources. AccaSim is thus an attractive tool for conducting job dispatching research in HPC systems.

==> sections/bio.tex <==
\begin{authorbiography}{%../authors/author.eps
}{Cristian Galleguillos}\
is a Ph.D. student under joint supervision at Pontificia Universidad Cat\'{o}lica de Valpara\'{i}so (PUCV), Chile and University of Bologna, Italy. He received his M.Sc. and Bachelor degrees in Computer Engineering from PUCV. His research interests include Constraint Programming, metaheuristics, and hybrid approaches for solving optimization problems.
\end{authorbiography}

\begin{authorbiography}{%../authors/author.eps
}{Zeynep Kiziltan}\
obtained her PhD degree in Computer Science from the University of Uppsala, Sweden, in 2004 with a thesis that won the European Coordinating Committee for Artificial Intelligence's Best PhD Dissertation Award. From 2004 to 2006 she worked at the University of Bologna as a post-doctoral researcher. In 2006 she was appointed Associate Professor by the University of Uppsala. Since 2006 she works as an Assistant Professor at the University of Bologna. Her research interests are in Artificial Intelligence, with a focus on Constraint Programming and its integration with Heuristic Search, Machine Learning and Data Science.
\end{authorbiography}

\begin{authorbiography}{%../authors/author.eps
}{Alessio Netti}\
is a research fellow at the Department of Computer Science and Engineering - University of Bologna. In 2017, he has acquired his M.Sc. title in Computer Science at the University of Bologna. In 2014, he has been an intern at the Italian Aerospace Research Center. His research interests range from HPC systems, to machine learning and signal processing. 
\end{authorbiography}

\begin{authorbiography}{%../authors/author.eps
}{Ricardo Soto}\
is an Associate Professor and Head of the Computer Science Department at the Pontificia Universidad Cat\'{o}lica de Valpara\'{i}so, Chile. He received his PhD degree in Computer Science from the University of Nantes, France, in 2009. His areas of research interest include mainly Metaheuristics, Global Optimization, and Autonomous Search. In this context, He has published about 180 scientific papers in different international conferences and journals, some of them top ranked in Computer Science, Operational Research, and Artificial Intelligence. Most of these papers are based on the resolution of real-world and academic optimization problems related to industry, manufacturing, rostering and seaports. 
\end{authorbiography}
